Giant catalytic effect of altruists in Schelling's segregation model

We study the effect of introducing altruistic agents in a Schelling-like model of residential segregation. We find that even an infinitesimal proportion of altruists has dramatic catalytic effects on the collective utility of the system. Altruists provide pathways that move the system away from the suboptimal equilibrium it would reach if the system included only egoist agents, allowing it to reach the optimal steady state.

==> reply.tex <==
dear Editor,

We are grateful for your message and the two reviews, which have helped us to improve in two major ways the manuscript: (a) the theoretical understanding of the transition and (b) the specific novelty of our work. Therefore, this new version satisfies the two main concerns of referee B.

Regarding (a), we have run new simulations to study in more detail the transition, showing that it is continuous. More important, we now present a theoretical analysis of the transition that {\it quantitatively} reproduces the simulation results without any free parameter. Concerning (b), we have carefully read the bibliography suggested by both referees and we are able to be more specific about the novelty of our work. It combines two important themes for many disciplines, including physics and economics: The large effects of small perturbations and the influence of altruistic behavior on coordination problems. We show that, unexpectedly, an infinitesimal proportion of altruists can coordinate a large number of egoists and allow the whole system to reach the social optimum. We have entirely rewritten the introduction and large parts of the discussion along these lines.

As we discuss in more detail below, in none of the suggested references we have found a model that shows such a giant catalytic effect produced by genuine altruist agents. For example, in the most similar work (by SS Liaw), a small proportion of agents is able to change the macroscopic properties of the system, but these agents have an artificially {\it fixed} behavior, which cannot properly be called "altruistic", as they do not sacrifice their own utility. Instead, in our work, agents do follow their own logic as real altruists (i.e. improving the utility of other agents) and the result emerges without deciding by hand that some agents should behave in a fixed manner.

As Referee A was positive and we have successfully addressed the two main concerns of Referee B, we feel that our revised article matches Phys Rev Lett standards. We attach to this letter a detailed reply to all referees' criticisms and the revised manuscript.

Best regards, Pablo Jensen -- corresponding author


***********
Referee A

This model exemplifies a very important social process and emphasizes the relevance of 
altruistic behavior in human societies. I think that this work will 
motivate further interesting studies. In sum, I suggest the 
publication of this work after taking into consideration the following 
remarks in the revision. 

R: We thank the referee for her/his positive evaluation of our manuscript,
and for the suggested references.

1) In the field of evolutionary game theory there are hundreds of 
papers studying the importance of altruistic behavior which is also a 
fundamental element in the Darwinian evolution (see the books by 
Maynard Smith, or Maynard Smith and Szathmary). In the evolutionary 
games the low utility of the society is generally caused by the pair 
interaction (represented by social dilemma games) between the selfish 
players and the "tragedy of the commons" can be avoided by the 
application of several types of altruistic behavior. Examples are 
models incorporating other-regarding preference or fraternal behavior 
(see e.g., Hetzer and Sornette, PLoS ONE 8 (2013) e77041; Szabo et al. 
J. Theor. Biol. 317 (2013) 126) and altruistic punishment (Fehr and 
Gachter, Nature (2002) 137; Boyd et al. PNAS 100 (2003) 3531; ..., 
Cong et al. Sci. Rep. 7 (2017) 14015). I think that the scientific 
value of this work can be increased significantly by drawing a 
parallel between the above-mentioned phenomena and the present one. At 
the same time the authors can emphasize the relevant differences and 
novelties. 

R: As noted above, these references have been very helpful to improve our knowledge of this subfield and understand that our model is important to understand the influence of altruistic behavior on coordination problems. We now include these references in the manuscript.

2) In the light of the previous results I suggest revising the last 
paragraph.

R: We have rewritten the last paragraph along these lines.

3) The readers can be helped by indicating the equivalence of the 
phrases "block" and "neighborhood".

R: This has been done.

----------------------------------------------------------------------
Report of Referee B -- LM16156/Jensen
----------------------------------------------------------------------

The manuscript "A simple model showing macroscopic effects of 
microscopic causes'" by Jensen et al. tackles the issue of introducing 
altruist agents in the Schelling segregation model. The paper is 
overall well written but there are several issues that preclude me 
from recommending publication in PRL. Most importantly, I am 
unconvinced of the novelty of the results and the execution also 
requires several revisions. 

In order in the manuscript: 

1) The title is vague and generic. A large fraction of "complex 
systems" articles published in PRE and PRL deal with systems that 
undergo phase transitions; i.e., where a microscopic variation can 
have macroscopic consequences. The title should do a much better job 
at describing the content of the manuscript. 

R: we agree : The title has been changed to "Giant catalytic effect of altruists in Schelling's segregation model" to be more precise about our work.

2) Minor comment: I would avoid using qualitative such as "celebrated" when presenting a model and/or reference. 

R: this word has been deleted

3) and 4) The authors say that their model challenges the intuition that 
"introducing a vanishingly small concentration of different agents 
should not change too much the collective state." What is this 
intuition based on? Most models of complex systems that are similarly 
based on game theory do have different phenomenology when a 
microscopic number of new agents with new behavior are introduced... 

R: We agree with the remark and thank the referee for pointing out these relevant articles. As stated above, her/his (and Referee A) remarks have made us realize that the novelty of our approach is not on the macro effect of a micro cause, but on the combination of two important themes: The large effects of small perturbations and the influence of altruistic behavior on coordination problems. We show that, unexpectedly, an infinitesimal proportion of altruists can coordinate a large number of egoists and allow the whole system to reach the social optimum.

5) The authors do cite the paper "Competition between collective and 
individual dynamics", which shares two authors with present 
manuscript. That paper also considers cooperativity as a form of 
altruism by using agents with consideration of the global welfare. I 
wish the authors better explained the important differences between 
their previous work and this manuscript. 

R: the important difference with our previous work is the {\it heterogeneity} of the population composition. In the PNAS paper, only pure populations were considered, with a homogeneous degree of egoism/altruism. We explain this point more precisely in the new version : "In \cite{pnas}, we have computed analytically the stationary states of a {\it homogeneous} population of egoist or altruist agents." We also discuss the importance of heterogeneity in the new discussion.

6) Figure 2 is interesting but the authors should run a lot more 
simulations to get better statistics. Right now the transition is so 
noisy that it is even hard to tell whether it is continuous or 
discontinuous. 

R: We have run new simulations to show that the transition is continuous (see the new Figure 2).

7) The presentation of the transition is also lacking. Are we dealing 
with a phase transition from a frustrated phase to a relaxed (globally 
optimal) phase? Or is utility simply monotonously rising with the 
number of altruists? A mean-field description alone could help 
understand the nature of this system in its thermodynamic limit(s). 

R: we now present a detailed theoretical argument to describe the transition, see Eq.(6) and the corresponding paragraph. Our scaling quantitatively fits the continuous transition of the average utility when altruist concentration increases.

8) Regarding Figure 4, I understand that this is an effective utility 
function which is useful as a thought experiment. But this one is 
drawn by considering the density of the neighborhood where altruistic 
agents are moving *to*, but the true utility is also a function of the 
density of the neighborhood they are moving *from*. In fact, the 
latter is probably more important since altruistic agents are likely 
to leave neighborhoods of high density for neighborhoods of low 
density, such that there are more residents affected by their move in 
the old neighborhood than in the new one. This means that they can 
still have a positive effective utility when moving to neighborhoods 
of density greater than 1/2. 

R : We believe that this specific comment results from a confusion on the definition and meaning of what we have called the "effective utility function u_{altr}(\rho)", which indicates that the introduction of this notion was not clear enough in the previous version of the manuscript. Let us first emphasize that the definition of u_{altr}(\rho) results from an exact mapping, and is by no means an approximation which would neglect some of the effects of a given move.

The idea is to reformulate in an exact way the dynamics of altruists as a selfish dynamics with a different individual utility function u_{altr}(\rho). This implies that when an agent moves, Delta U = Delta u_{altr}(\rho).
In other words, the variation of the total utility U = sum_i u(rho_i) can be re-expressed as the variation of an individual utility u_{altr}(\rho) between the initial and final blocks. This is not a priori obvious, but this builds on the results of Ref.[4], where the variation of the individual utility u(rho) was shown to be equal to the variation of a function L = sum_q l(rho_q) of the full configuration of the model. The local function l(rho) in each block is equal to rho*u(rho) for an altruist dynamics, and to int_0^rho u(rho') d rho' for an egoist dynamics. To map the altruist dynamics onto an egoist one, we thus define u_{altr}(\rho) such that rho*u(rho) = int_0^rho u_{altr}(\rho') d rho', see Eq.(1), which yields the explicit expression Eq.(2) of u_{altr}(\rho) by derivation.

9) I'm confused by the subsection "Dependence on system's size Q". 
First of all because the thermodynamic limit can be defined both in 
terms of Q or H. Second of all because the authors use the phrase "to 
prove this point" but end up providing only a very soft illustration 
(with several assumptions) of why it might be correct, rather than a 
proof that it is. 

R: We agree that the term "prove" was an overstatement. We now provide precise arguments showing that there is a continuous transition on the average utility. Having better formalized our arguments, we are now able to derive an explicit formula for the average utility as a function of the fraction p of altruists, in the regime where this fraction is very small, of the order of 1/Q. Concerning the thermodynamic limit, we focus on the limit where the number of blocks goes to infinity. The maximal number H of agents in each block is taken to be large from the outset, so that one can define a continuous density in each block.

10) I'm afraid the physical analogies in the discussion did not really 
provide me with much additional insights. The model is simple enough 
and the paper is already clearly written. However, I would disagree 
that the model illustrates "extreme sensitivity" to a system's 
composition. In fact, except in an extremely narrow region of 
parameter space, the model does not respond at all to a change in 
frequency of altruism. Moreover, even around the transition we are 
facing a continuous answer function: a microscopic change in p appears 
to lead to a continuous change in average utility (unless gathering 
more statistics on Fig 2 ends up highlighting a discontinuous 
transition). In fact, I thought the authors were going to discuss the 
nature of the transition after Eq. (3) but the discussion ended up 
very confusing. The susceptibility does not diverge (not shown) but 
has a singularity. What is meant by singularity? 

R: We agree that the discussion in the first version of the manuscript was confusing. We have rephrased it to provide clarifications. As mentioned above, we are now able to provide a mathematical argument pointing to a continuous transition, with a good match with numerical data. We also agree that the term "singularity" was somehow confusing. By this we meant that a discontinuity in the second derivative of the "free energy" may already be thought of as a singularity. However, this may not be very relevant as this was a property of the model with egoists only. We have removed from the discussion the few unclear sentences related to this point.

As for the "extreme sensitivity", we understand the referee's viewpoint that the sensitivity is not present for any fraction of altruists, but only in the limit of a very small fraction. We now rather speak of a giant catalytic effect, to emphasize that a very small fraction of altruists leads to a strongly amplified macroscopic response through a catalytic effect, in the sense that altruists are not "consumed", but can successively help egoists fill up some blocks many times.

11) Several references could be added to provide context to this work 
since it certainly does not exist in a vacuum. The authors currently 
mostly cite their work on the subject but ignore several other models 
with similar phenomenology and even similar mechanisms (such as the El 
Farol game mentioned above).

R: we agree and have enriched the bibliography (see points 3 and 4 above)
